ICSFuzz: Collision Detector Bug Discovery in Autonomous Driving Simulators

With the increasing adoption of autonomous vehicles, ensuring the reliability of autonomous driving systems (ADSs) deployed on autonomous vehicles has become a significant concern. Driving simulators have emerged as crucial platforms for testing autonomous driving systems, offering realistic, dynamic, and configurable environments. However, existing simulation-based ADS testers have largely overlooked the reliability of the simulators, potentially leading to overlooked violation scenarios and subsequent safety security risks during real-world deployment. In our investigations, we identified that collision detectors in simulators could fail to detect and report collisions in certain collision scenarios, referred to as ignored collision scenarios. This paper aims to systematically discover ignored collision scenarios to improve the reliability of autonomous driving simulators. To this end, we present ICSFuzz, a black-box fuzzing approach to discover ignored collision scenarios efficiently. Drawing upon the fact that the ignored collision scenarios are a sub-type of collision scenarios, our approach starts with the determined collision scenarios. Following the guidance provided by empirically studied factors contributing to collisions, we selectively mutate arbitrary collision scenarios in a step-wise manner toward the ignored collision scenarios and effectively discover them. We compare ICSFuzz with DriveFuzz, a state-of-the-art simulation-based ADS testing method, by replacing its oracle with our ignored-collision-aware oracle. The evaluation demonstrates that ICSFuzz outperforms DriveFuzz by finding 10-20x more ignored collision scenarios with a 20-70x speedup. All the discovered ignored collisions have been confirmed by developers with one CVE ID assigned.

==> input/07_caseStudy.tex <==
% \newpage


\begin{figure}[!ht]
% \begin{minipage}[b]{\linewidth} 
\centering
\includegraphics[width=\linewidth]{fig/case_study_flb.pdf} 
\caption{case study.}
\label{fig:case_study}
\end{figure}


\section{\textcolor{red}{Case Study}}
% use the case in flb, as the condition shown in motivating example
\textbf{ICS 01}:
As shown in Figure~\ref{fig:case_study}, a clear collision occurred from \texttt{t2}, and the NPC bicycle was knocked down by the vehicle at \texttt{t3}. After the EV departs, the NPC bicycle falls to the ground (\texttt{t4}), resulting in significant damage. 
Notably, the collision detector failed to report the incident throughout the entire sequence.

\textbf{Safety Consequences}:
If an ADS encounters this collision scenario during testing or development in the simulator, it may prevent the ADS developers from identifying and making necessary improvements to the system. Consequently, when the same ADS is deployed in the real world and encounters similar environmental conditions, it could make the same erroneous decision, potentially leading to a real collision with a cyclist. 
Such incidents could result in severe injuries or even fatalities for the cyclist. 

The potential consequences underscore the critical need for robust collision detection mechanisms in the simulator to ensure the safety and reliability of ADS during testing and development, ultimately safeguarding real-world applications.


==> input/backup_intro.tex <==
%% 
\wei{updated paragraphs-wei}
Given the complexity and difficulty of deploying Autonomous Driving (AD) in real-world scenarios, 
AD simulators have become the most commonly used development and testing platform in the rapid development and iteration of Autonomous Driving Systems (ADS) such as Autoware~\cite{autoware} and Baidu Apollo~\cite{apollo}. 
Following industrial and academic practice, ADS are first strictly tested inside simulators like Carla~\cite{carla} to ensure their robustness and reliability and then equipped on physical vehicles for further road testing. 
Similarly, many advanced autonomous driving algorithms are also developed and heavily tested upon simulators before being ported to ADS. 
%For example, collision detectors (or collision detection algorithms) for autonomous driving, one of ADS's most fundamental functional components, are usually tested inside simulators with diverse settings and safety considerations before being permitted to be integrated into ADS. 
Such careful testing conventions result from numerous life and accident losses during real-world collision accidents. 
The data of the National Highway Traffic Safety Administration Crash Report Sampling System (NHSTA CRSS)~\cite{nhsta_crss} shows that millions of collisions happen yearly. 
In 2021, there were 6.1 million collisions happened in the USA, of which nearly 40000 resulted in a death~\cite{nhsta_2021_collision_reports}. %maybe give the data of ADS accidents
Thus, many existing works tried to detect any potential collisions in the early stage of ADS or detection algorithm development with a convention of adopting AD simulators' built-in collision detector as the testing oracle~\cite{avfuzzer,avchecker,planfuzz,drivefuzz}.

However, the existing test works all focus on ADS security and ignore the correctness of the underlying simulator, especially the correctness of the built-in collision detector within the simulator. 
We observed the collision detector in simulators sometimes malfunctioned or failed, and defined it as \textit{collision detection inconsistency}(CDI). 
The CDI occurs when the collision detector should have reported a collision event but failed to do so..
The aforementioned previous works essentially attempt to find "collision and detected" scenarios. 
their oracle was unable to find the CDI scenarios we are looking for since using the built-in collision detector as the oracle in simulator testing to identify issues within the oracle itself is self-contradictory. 


\begin{figure}[htbp]
  \begin{minipage}[b]{\linewidth} 
    \centering
    \includegraphics[width=\linewidth]{fig/collision_noncollision_space.pdf} 
    % \subcaption{Collision and Non-collision space. A: Existing works run with their oracle. B: Existing works run with suitable CDI oracle C: Our Method. } 
    \label{fig: motivating: collision and non-collision space}
  \end{minipage}
  \caption{Motivating example: Collision and Non-collision space illustration in 2D space. A: Existing works run with their oracle. B: Existing works run with suitable CDI oracle. C: Existing works run with suitable CDI oracle without accurately located to CDI space.  D: Existing works with less randomness. E: Our Method.} 
  % (a) Collision and successfully detected scene (b) No collision scene (c) Illustration of collision and Non-collision space  
  \label{fig: motivating example}
\end{figure}


%efficiency
Two additional significant challenges make it difficult to directly apply existing simulation-based ADS testing approaches for testing CDI events.
First, as condition A shown in Figure \ref{fig: motivating example}, existing approaches typically start from the non-collision space and eventually reach a point in the collision space, aiming to generate diverse corner cases for testing ADS. 
To achieve this, they intentionally introduce randomness, which brings a lot of computation overhead in the non-collision space.
However, to find the CI events, the fuzzer needs to get to the collision space as fast as possible and find the CI events around the collision space. 
When conducting corner case testing for ADS, the additional computations become valuable because they introduce unintended scenarios.  
In CDI testing, the excessive randomness introduced by existing approaches hinders the speed of CDI scenario discovery. 
In this context, the additional computations become less valuable as they do not contribute effectively to the detection of CDI events.

%accuracy
Second, even with guided fuzzing and the replacement of the oracle with a CDI-capable oracle, it is common to bypass the CDI space and directly reach the collision space. 
This is primarily due to the small size of the CDI space and its proximity to the collision space. 
As shown in Figure \ref{fig: motivating example}, condition B is what we want, but it is highly likely to be condition C. 
As shown in Figure \ref{fig: motivating example}, condition B represents the ideal scenario where CDI events are precisely located and explored.
However, it is highly likely to end up in condition C, where the CDI space is bypassed.
This results in reduced accuracy in testing for testing for CDI events.


To address the aforementioned problems, our key insight is that the fuzzer can decrease the level of randomness within the non-collision space and precisely determine the boundaries of the CDI space, increasing both the efficiency and accuracy of CDI event detection. 
\begin{itemize}
    \item Reducing randomness in the non-collision space because the primary objective is to quickly identify collision scenarios and promptly detect CDI events around them.
    By minimizing randomness, the fuzzer can focus on generating test scenarios that are closer to CDI space, which helps speed up the discovery of CDI events.
    For example, if the seed scenario is the one shown in Figure \ref{fig: motivating example}, condition D saves more time than conditions A, B, and C in reaching the target space.
    \item Precisely locating the boundaries of the CDI space is also essential, which ensures the final testing destination of the fuzzer falls within the critical area.
    As shown in Figure \ref{fig: motivating example}, condition B is the desired outcome instead of condition C.
    Furthermore, localizing the boundaries of the CDI space opens up possibilities for further exploration within its interior, enabling a more comprehensive analysis of CDI events.

\end{itemize}




\zk{summarize the technical challenges of \sysname in a numbered list. e.g., 1) ... 2) ... 3) ...}

Based on these insights, in this paper, we propose \sysname, 
an asymptotic reverse end-to-end approach for testing CDI in AD simulators. 
To the best of our knowledge, \sysname is the first work focusing on the security of ADS simulators.
We first precisely localize the boundaries of the CDI space, distinguishing between those adjacent to the collision space and those adjacent to the non-collision space separately.
Then we initiate guided fuzzing testing from the collision space, setting the destination as the non-collision space and proceeding in reverse, as shown in condition E in Figure\ref{fig: motivating example}.
This reverse testing strategy allows for better exploration of the CDI space and the identification of conditions and potential reasons for collision detector failure. 
o achieve comprehensive testing within the CDI space, a step-by-step approach is employed to systematically modify scenario parameters.


We implement \sysname on Carla~\cite{carla}, a widely used autonomous driving simulator based on Unreal Engine. 
We compare \sysname with DriveFuzz~\cite{drivefuzz}, a state-of-the-art simulation-based fuzzer. 
To enable Drivefuzz to detect CDI events, we replaced its oracle with a CDI-capable oracle. 
Through the exploration of the CDI space and the discovery of CDI events, the underlying factors contributing to their occurrence are identified.
We reported the CDI events to AD simulator developers and feedback was obtained from community users who have experienced similar issues.
\wei{supplement the comparison result, factors relationship later}

In summary, this paper makes the following contributions: 
\zk{update the following bullet points w/ more defining but convincing words.}
\begin{itemize} 
    \item We propose an end-to-end black-box generic testing approach to systematically identify collision detection inconsistency bugs within AD simulators. 
    \item  We design a novel approach for generating test cases that aim to uncover CDI events across various scenarios. The identification of CDI events allows for the attribution of factors contributing to their occurrence. 
    \item We implement and evaluate a prototype named \sysname. The evaluation result shows xx\% CDI events were found. Also, from the result, we found a relationship between CDI events and different environment parameters like collision speed, angle, and participant type. The relationship helps us estimate the collision detector's underlying logic and corresponding thresholds in CARLA. 
    \zk{to be refined}
    \wei{1.supplement the data and method detail later with experiment results 2. define scenario and scene in paper}
\end{itemize}






==> input/float_figs/fig_MotivatedExampleAndProblemSpace.tex <==
%%
\begin{figure}[tp]
% \begin{minipage}[b]{\linewidth} 
\centering
%%
\begin{subfigure}{1.0\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/scenario_illustration.pdf} 
\caption{
Scenario Illustration: Three different vehicle relationships of scenario \texttt{FollowLeadingBicycle} in AD simulator Carla~\cite{carla}. 
% The right side is the abstract relationship between collision and non-collision events of the scene shown on the left.
$A$: no collision happened while the vehicle and bicycle were out of contact. 
$B$: CDI event. The vehicle crashed with the bicycle, but collision sensors attached to both the vehicle and the bicycle failed to report the collision case. 
$C$: a collision but detected event; the collision happened, and the collision sensor successfully reports the collision event. 
% \zk{TDOO: move the caption of each subfigure to their subcaption.}
}
\end{subfigure}

%%
\begin{subfigure}{1.0\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/search_space.pdf} 
\caption{Search space.
Collision Space encompasses all collision events.
Collision Detection Inconsistency(CDI) Space encompasses all CDI events.
ADS Collision Space encompasses the collision events caused by the ADS failure.
ADS collision events and CDI events exist as specific cases of collision events within the collision space. 
The ADS collision space and CDI space intersect but do not completely overlap.
Outside of the collision space, a well-defined non-collision space exists.
A: Existing ADS testers focus on multiple violations.  B: Existing ADS testers focus on collisions only. C: Our Method: Start from a determined collision case and use pre-studied search direction and searching step.
In conclusion, our method is better suited for the specific simulator safety problem, it enables a higher efficiency and a greater likelihood of identifying CDI events.}
\end{subfigure}
%%
\caption{
TODO. 
}
\label{fig:motivating example}
\end{figure}

==> input/float_figs/fig_Overview.tex <==
%%
% \captionsetup{labelfont=bf}
% \captionsetup{font=bf}
\begin{figure}[tp]
\centering
\includegraphics[scale=0.25]{fig/system_structure.pdf}
\caption{\S~\ref{sec:overview}: Overview of \sysname. 
1) Offline stage. % (\S~\ref{sec:design:offline}). % Detected collision scenarios collection by empirical study. 
Determining detected collision scenarios, searching direction and step size through empirical study. 
2) Online stage. % (\S~\ref{sec:design:online_stage}). 
Fuzzing test AD simulator for IC bugs. 
}
\label{figure:system_structure}
\end{figure}

==> input/float_figs/fig_Pipeline.tex <==
%%
\captionsetup{labelfont=bf}
\captionsetup{font=bf}
\begin{figure}[tbp]
\centering
\includegraphics[scale=0.25]{fig/system_structure.pdf}
\caption{Overview of \sysname.}
\label{figure:system_structure}
\end{figure}

==> input/float_figs/fig_ScenariosIllustration.tex <==
%%
\begin{figure}[tp]
% \begin{minipage}[b]{\linewidth} 
\centering
\includegraphics[width=\linewidth]{fig/scenario_illustration.pdf} 
\caption{
Scenario Illustration: Three different vehicle relationships of scenario \texttt{FollowLeadingBicycle} in AD simulator Carla. 
%The right side is the abstract relationship between collision and non-collision events of the scene shown on the left.
$A$ represents that no collision happened while the vehicle and bicycle were out of contact. 
$B$ is a CDI event, the vehicle crashes with the bicycle, but collision sensors attached to both the vehicle and the bicycle failed to report the collision case. 
C is a collision but detected event, the collision happened and the collision sensor successfully reports the collision event.
%Route 1 represents the ideal situation adopting existing works with a CDI-oriented oracle on CDI event detection. 
%Route 2 represents the actual situation adopting updated works, skipping the CDI event, and directly generating the collision event for testing.
%Route 3 is our method, starting from the position close to the collision space and running reverse testing. 
}
\label{fig:motivating example}
\end{figure}


==> input/float_figs/fig_SearchSpace.tex <==
\begin{figure}[tp]
\centering
\includegraphics[width=\linewidth]{fig/search_space.pdf} 
\caption{Search space.
CD space: Collision and Detected Space. 
CDI space: Collision Detection Inconsistency Space.
A: Existing ADS tester without CDI-guided mutation strategy.  
B: Existing ADS tester with a CDI-guided mutation strategy.
C: Our Method: Start from the CD space and stop at the CDI space with an incrementally CDI-guided mutation strategy.\huang{add conclusion}}
\label{fig:search_space}
\end{figure}

==> input/float_figs/fig_SimulatorStructure.tex <==
%% 
\begin{figure}[tp]
\centering
\includegraphics[width=\linewidth]{fig/simulator_structure.png} 
\caption{Structure of AD simulator} 
\label{fig:simulator structure}
\end{figure}

==> input/float_figs/fig_bg_simulator.tex <==
%% 
\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{fig/simulator_structure.png} 
\caption{
Structure of AD simulator.} 
\label{fig:simulator structure}
\end{figure}

==> input/float_figs/fig_eval_DriveFuzz_AverageTime_Comparison.tex <==
% %%
% \begin{figure}[tp]
% \centering
% % \includegraphics[width=1\linewidth]{fig/drivefuzz_time.png}
% \includegraphics[width=0.8\linewidth]{fig/result/DriveFuzz_comparison/average_time_comparison.png} 
% \caption{AVerage Time taken by Drivefuzz and \sysname to find three types of UC events. 
% The y-axis represents the time in hours.}
% \label{fig:drivefuzz_ave_time}
% \end{figure}


% \begin{figure}[tp]
% \centering
% % \includegraphics[width=1\linewidth]{fig/drivefuzz_time.png}
% \includegraphics[width=0.8\linewidth]{fig/result/DriveFuzz_comparison/average_time_comparison_hist.png} 
% \caption{AVerage Time taken by Drivefuzz and \sysname to find three types of UC events. 
% The y-axis represents the time in hours.}
% \label{fig:drivefuzz_ave_time_hist}
% \end{figure}




\begin{figure}[tp]
\centering
% \includegraphics[width=0.6\linewidth]{fig/result/DriveFuzz_comparison/DriveFuzz_times.png} 
\includegraphics[width=0.6\linewidth]{fig/result/DriveFuzz_comparison/Drivefuzz_ratio_radar.png} 

\caption{\S~\ref{sec:eval:rq2_search_space}: The average time and proportion ratio between DriveFuzz and UCfuzz for three types of UC events. 
The time ratio indicates how often the average time DriveFuzz takes to discover an event within a specific class exceeds the average time taken by \sysname.
The proportion ratio represents how much the proportion of UC events discovered by \sysname exceeds the proportion of UC-prone events discovered by DriveFuzz. 
%\zk{a little bit long.}
}
\label{fig:drivefuzz_ave_times}
\end{figure}

==> input/float_figs/fig_eval_DriveFuzz_TimeCost.tex <==
%%
\begin{figure}[tp]
\centering
% \includegraphics[width=1\linewidth]{fig/drivefuzz_time.png}
\includegraphics[width=0.5 \linewidth]{fig/result/DriveFuzz_comparison/Drivefuzz-box-log.png} 
\caption{\S~\ref{sec:eval:rq2_search_space}: Time taken by Drivefuzz and \sysname to find UC events. 
DriveFuzz identified  12 UC events, we compare the search time for the same set of 12 UC events found in \sysname.
The y-axis represents the time, which has been uniformly converted to minutes and then logarithmically scaled to achieve better visualization.}
\label{fig:drivefuzz_time}
\end{figure}

==> input/float_figs/fig_eval_IC_SR_CollisionAngle.tex <==
\begin{figure}[tp]
    \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_angle/angle-line-FLB.png}
    \caption{Follow Leading Bicycle}
    \label{fig:sr_angle-flb}
    \end{subfigure}
\hfill
    \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_angle/angle-line-FLV.png}
    \caption{Follow Leading Vehicle}
    \label{fig:sr_angle-flv}
    \end{subfigure}
% \vspace{1em}
    \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_angle/angle-line-PSF.png}
    \caption{Pedestrian Standing Front}
    \label{fig:sr_angle-psf}
    \end{subfigure}
\hfill
    \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_angle/angle-line-LC.png}
    \caption{Lane Change}
    \label{fig:sr_angle-lc}
    \end{subfigure}
% \vspace{1em}
    \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_angle/angle-line-PCF.png}
    \caption{Pedestrian Crossing Front}
    \label{fig:sr_angle-pcf}
    \end{subfigure}
\hfill
    \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_angle/angle-line-InC.png}
    \caption{Intersection Collision}
    \label{fig:sr_angle-inc}
    \end{subfigure}
%% 
\caption{\S~\ref{sec:eval:rq3_search_direction}: ICS success rate with collision angle.}
\label{fig:IC_SR-angle}
\end{figure}


==> input/float_figs/fig_eval_IC_SR_CollisionDistance.tex <==
\begin{figure}[tp]
  \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_distance/distance-bar-FLB.png}
    \caption{Follow Leading Bicycle}
    \label{fig:sr_distance-flb}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_distance/distance-bar-FLV.png}
    \caption{Follow Leading Vehicle}
    \label{fig:sr_distance-flv}
  \end{subfigure}
  % \vspace{1em}
  \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_distance/distance-bar-PSF.png}
    \caption{Pedestrian Standing Front}
    \label{fig:sr_distance-psf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_distance/distance-bar-LC.png}
    \caption{Lane Change}
    \label{fig:sr_distance-lc}
  \end{subfigure}
  % \vspace{1em}
  \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_distance/distance-bar-PCF.png}
    \caption{Pedestrian Crossing Front}
    \label{fig:sr_distance-pcf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_distance/distance-bar-InC.png}
    \caption{Intersection Collision}
    \label{fig:sr_distance-inc}
  \end{subfigure}
\caption{\S~\ref{sec:eval:rq3_search_direction}: ICS success rate with collision distance.}
\label{fig:IC_SR-distan}
\end{figure}


==> input/float_figs/fig_eval_IC_SR_CollisionSpeed.tex <==
\begin{figure}[tp]
  \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_speed/speed-bar-FLB.png}
    \caption{Follow Leading Bicycle}
    \label{fig:sr_speed-flb}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_speed/speed-bar-FLV.png}
    \caption{Follow Leading Vehicle}
    \label{fig:sr_speed-flv}
  \end{subfigure}
  % \vspace{1em}
  \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_speed/speed-bar-PSF.png}
    \caption{Pedestrian Standing Front}
    \label{fig:sr_speed-psf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_speed/speed-bar-LC.png}
    \caption{Lane Change}
    \label{fig:sr_speed-lc}
  \end{subfigure}
  % \vspace{1em}
  \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_speed/speed-bar-PCF.png}
    \caption{Pedestrian Crossing Front}
    \label{fig:sr_speed-pcf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.19\textwidth}
    \includegraphics[width=\textwidth]{fig/result/single_feature_speed/speed-bar-InC.png}
    \caption{Intersection Collision}
    \label{fig:sr_speed-inc}
  \end{subfigure}
\caption{\S~\ref{sec:eval:rq3_search_direction}: ICS success rate with collision speed.}
\label{fig:IC_SR-speed}
\end{figure}


==> input/float_figs/fig_eval_RQ1_two.tex <==
\begin{figure}[t]
  \begin{subfigure}[t]{0.235\textwidth}
    \includegraphics[width=\textwidth]{fig/result/DriveFuzz_comparison/Drivefuzz-box-log.png}
    \caption{
    }
    \label{fig:eval:drivefuzz_time}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.235\textwidth}
    \includegraphics[width=\textwidth]{fig/result/DriveFuzz_comparison/ratio_radar.png}
    \caption{
    }
    \label{fig:eval:drivefuzz_ave_times}
  \end{subfigure}
    \caption{
    (a) Comparison of time taken to identify ICSs, logarithmically scaled.
    (b) Comparison of time and proportion ratio for three types of ICSs identified by DriveFuzz.
    \textcolor{red}{replace fig 9 with table 3?}
    }
\label{fig:eval:RQ2}
\vspace{-5mm}
\end{figure}

==> input/float_figs/fig_eval_Relationship1_CollisionDistance_with_Speed.tex <==



%%
\begin{figure}[tp]
  \centering
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_speed-with-distance/SR-distance-speed-FLB.png}
    \caption{Follow Leading Bicycle}
    \label{fig:sr-distance_speed_flb}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_speed-with-distance/SR-distance-speed-FLV.png}
    \caption{Follow Leading Vehicle}
    \label{fig:sr-distance_speed_flv}
  \end{subfigure}

  \vspace{1em}
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_speed-with-distance/SR-distance-speed-PSF.png}
    \caption{Pedestrian Standing Front}
    \label{fig:sr-distance_speed_psf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_speed-with-distance/SR-distance-speed-LC.png}
    \caption{Lane Change}
    \label{fig:sr-distance_speed_lc}
  \end{subfigure}

  \vspace{1em}
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_speed-with-distance/SR-distance-speed-PCF.png}
    \caption{Pedestrian Crossing Front}
    \label{fig:sr-distance_speed_pcf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.231\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_speed-with-distance/SR-distance-speed-InC.png}
    \caption{Intersection Collision}
    \label{sec:eval:multiple_factor}
  \end{subfigure}
\caption{\S~\ref{sec:eval:multiple_factor}: Relationship between ICS SR and Collision Speed at Different Collision Distance Scope.}
\label{fig:IC_SR-speed-distance}
\end{figure}







==> input/float_figs/fig_eval_Relationship1_CollisionSpeed_with_Distance.tex <==
%%
\begin{figure}[tp]
  \centering
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_distance-with-speed/SR-speed-distance-bar-FLB.png}
    \caption{Follow Leading Bicycle}
    \label{fig:sr-distance-speed_flb}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_distance-with-speed/SR-speed-distance-bar-FLV.png}
    \caption{Follow Leading Vehicle}
    \label{fig:sr-distance-speed_flv}
  \end{subfigure}

  % \vspace{1em}
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_distance-with-speed/SR-speed-distance-bar-PSF.png}
    \caption{Pedestrian Standing Front}
    \label{fig:sr-distance-speed_psf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_distance-with-speed/SR-speed-distance-bar-LC.png}
    \caption{LaneChange}
    \label{fig:sr-distance-speed_lc}
  \end{subfigure}

  % \vspace{1em}
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_distance-with-speed/SR-speed-distance-bar-PCF.png}
    \caption{Pedestrian Crossing Front}
    \label{fig:sr-distance-speed_pcf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_distance-with-speed/SR-speed-distance-bar-InC.png}
    \caption{Intersection Collision}
    \label{fig:sr-distance-speed_inc}
  \end{subfigure}
  \caption{\S~\ref{sec:eval:multiple_factor}: Relationship between ICS SR and Collision Distance at Different Collision Speed Scope.}
  \label{fig:IC_SR-distance-speed}
\end{figure}


==> input/float_figs/fig_eval_Relationship2_CollisionAngle_Speed.tex <==
\begin{figure}[tp]
  \centering
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_speed-angle/SR-speed-angle-line-FLB.png}
    \caption{Follow Leading Bicycle}
    \label{fig:sr-speed-angle-flb}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_speed-angle/SR-speed-angle-line-FLV.png}
    \caption{Follow Leading Vehicle}
    \label{fig:sr-speed-angle-flv}
  \end{subfigure}

  % \vspace{1em}

  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_speed-angle/SR-speed-angle-line-LC.png}
    \caption{Lane Change}
    \label{fig:sr-speed-angle-lc}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_speed-angle/SR-speed-angle-line-PSF.png}
    \caption{Pedestrian Standing Front}
    \label{fig:sr-speed-angle-psf}
  \end{subfigure}

  % \vspace{1em}

  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_speed-angle/SR-speed-angle-line-PCF.png}
    \caption{Pedestrian Crossing Front}
    \label{fig:sr-speed-angle-pcf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_speed-angle/SR-speed-angle-line-InC.png}
    \caption{Intersection Collision}
    \label{fig:sr-speed-angle-inc}
  \end{subfigure}
\caption{\S~\ref{sec:eval:multiple_factor}: Relationship between ICS SR and Collision Angle at Different Collision Speed Scope.}
  \label{fig:IC_SR-speed-angle}
\end{figure}



==> input/float_figs/fig_eval_Relationship3_CollisionAngle_Distance.tex <==
%%
\begin{figure}[tp]
  \centering
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_distance-angle/SR-distance-angle-FLB.png}
    \caption{Follow Leading Bicycle}
    \label{fig:sr-dist-angle-flb}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_distance-angle/SR-distance-angle-FLV.png}
    \caption{Follow Leading Vehicle}
    \label{fig:sr-dist-angle-flv}
  \end{subfigure}
  % \vspace{1em}
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_distance-angle/SR-distance-angle-LC.png}
    \caption{Lane Change}
    \label{fig:sr-dist-angle-lc}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_distance-angle/SR-distance-angle-PSF.png}
    \caption{Pedestrian Standing Front}
    \label{fig:sr-dist-angle-psf}
  \end{subfigure}
  % \vspace{1em}
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_distance-angle/SR-distance-angle-PCF.png}
    \caption{Pedestrian Crossing Front}
    \label{fig:sr-dist-angle-pcf}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{fig/result/multi_feature_distance-angle/SR-distance-angle-InC.png}
    \caption{Intersection Collision}
    \label{fig:sr-dist-angle-inc}
  \end{subfigure}

  \caption{\S~\ref{sec:eval:multiple_factor}: Relationship between ICS SR and Collision Angle at Different Distance.}
  \label{fig:IC_SR-dist-angle}
\end{figure}


==> input/u_discussion.tex <==
% \newpage 

\section{Discussion}


\zk{TODO. Potential \& Limitations.}

Our intuition to effectively discover ICSs comes with a novel view of their correlation with other scenarios in the simulator. Our observation is that since
ICSs are the false negative results of the collision detector, which an ICS must be a collision scenario, they only exist in the $S$. 
Thus, slightly mutating the collision scenarios is more likely to transfer them into ICSs than non-collision scenarios. 

Based on these observations, our idea is to directly conduct the ICS discovery starting from $S$ 
with a selective mutation strategy targeting ICSs in a step-wise manner.
If we can only mutate the related factors that lead to ICSs, the effectiveness of input generation can be significantly improved with fewer irrelevant inputs generated.

1. Influential Scenario Collections via High-Frequency Collisions

2. Selective Scenario Mutation with Collision-Contributing Factors. 

==> input/x_acknowledgement.tex <==
% \newpage

% \section*{Acknowledgment}


% The authors would like to thank...

==> input/z_evaluation_ccs.tex <==
% \newpage 


%% rq1
\input{tables/tab_eval_IC_ICFuzz}



\section{Evaluation}
\label{sec:eval}
We implemented \sysname, a black-box fuzzer with a step-wise mutation approach starting from the collision space to find the ICSs in the AD simulator effectively.
We will release our code and prototype after the paper is accepted.
Based on the implementation, we design a series of evaluations to demonstrate the effectiveness of \sysname by investigating the following research questions:



%%
\begin{itemize}[leftmargin=*]
\item \textbf{RQ1:} Can \sysname effectively discover ICSs?
\item \textbf{RQ2:} Can \sysname efficiently discover ICSs starting from the collision scenario space?
\item \textbf{RQ3:} Can step-wise mutation generate ICSs effectively?
\item \textbf{RQ4:} Can \sysname precisely identify all detected ICSs?
\end{itemize}

To validate whether \sysname can effectively find ICSs compared to existing ADS testers (\textbf{RQ1}), we run a state-of-the-art ADS fuzzer, DriveFuzz, equipped with our ICS oracle to compare its ICS identification ability with \sysname in \S~\ref{sec:eval:rq1_drivefuzz_comparison}.
To validate our intuition that whether starting discovering from the collision scenario space is more efficient than from the non-collision scenario space (\textbf{RQ2}), we compare the discovery time and number of ICSs between DriveFuzz and \sysname in \S~\ref{sec:eval:rq2_search_space}.
Furthermore, we conduct ablations to validate whether the mutation strategy in \sysname can effectively detect ICSs (\textbf{RQ3}),  
we analyze the ICSs discovered by \sysname to discern the search directions in the final results and determine if they align with our designated approach in \S~\ref{sec:eval:rq3_search_direction}.
Finally, we study the precision of our oracle in indicating ICSs (\textbf{RQ4}). We vary the threshold values of the oracle to investigate their impact on the precision and recall in \S~\ref{sec:eval:rq4_oracle-threshold}.


\textbf{Benchmark.} The simulator used for testing in this study is Carla, one of the most widely used autonomous driving simulators.
While various types of driving simulators exist, some are proprietary and charged, such as PreScan~\cite{prescan}.
On the other hand, other simulators primarily focus on traffic flow simulation and lack a realistic 3D environment, such as SUMO~\cite{sumo} and WayMax~\cite{waymax}.
Among the available options, LGSVL~\cite{lgsvl} and Carla~\cite{carla} provided a 3D realistic environment and multiple APIs for different ADS, such as AutoWare~\cite{autoware}, Apollo~\cite{apollo}.
However, LGSVL has suspended active development as of January 1, 2022.
Therefore, this paper focuses on testing the latest stable version of Carla (0.9.13).


\textbf{Baseline.} 
% \zk{TODO.} 
% \huang{why only Drivefuzz} 
The majority of simulation-based ADS testers do not make their project code open-source.
Among the open-source projects, LGSVL was used in most of them to test Apollo before 2022, but unfortunately, they are outdated along with LGSVL.
DriveFuzz~\cite{drivefuzz} and ADFuzz~\cite{ADfuzz} use Carla as the testing platform and are open-source.
However, ADFuzz does not employ Carla's docker version, which cannot run on a server.
Meanwhile, we have contacted the authors of ADFuzz. Unfortunately, this tool is not maintained anymore. 
In contrast, DriveFuzz provided a docker version for evaluation.
Therefore, we choose DriveFuzz\cite{drivefuzz} as our baseline.

% DriveFuzz utilizes multiple indicators, including the ratio of hard acceleration, lateral force, and the minimum distance to the closest NPC, to form as the fitness function.
% Based on the fitness value of each testing round, DriveFuzz generates new NPCs or puddles near the tested autonomous vehicle in the simulator to mutate scenarios with higher danger levels.

\textbf{Configuration.} We conducted the evaluation on the server machine running Ubuntu20.04, powered by 80-core Intel Xeon Gold 6242R CPU, 188 GB memory, and 2 Nvidia A30 graphics cards. 
% \clearpage


% \textbf{Metric.} We utilize the ICS success rate as our metric to quantify the total number of ICSs ratio in all generated collision scenarios. 

%%
\subsection{\textbf{RQ1:} Can \sysname Effectively Discover ICSs?}
\label{sec:eval:rq1_drivefuzz_comparison}

%% RQ2
\input{input/float_figs/fig_eval_RQ1_two}
\input{tables/tab_eval_comparison_ratio}

The main goal of \sysname is to discover all ICSs efficiently.
Thus, we first compare \sysname with the state-of-the-art ADS fuzzer DriveFuzz.
We run each fuzzer for $36$ hours and compare the number of discovered ICSs, the respective collision types, and the time spent to discover them.
Since the default collision detector used by DriveFuzz cannot identify ICSs, we replace it with an IC-capable oracle, as discussed in \S~\ref{sec:overview}, for a fair comparison.

The results are shown in Table~\ref{tab:discovered_ICs}, which lists all types of ICSs found by the \sysname, along with the corresponding values of control parameters and collision factors.
DriveFuzz only discovers 12 ICSs in 3 ICS categories, as listed in Table~\ref{tab:discovered_ICs}.
Instead, \sysname successfully discovers 473 ICSs covering ten types of ICSs.
Meanwhile, DriveFuzz requires 0.28 to 5 hours to discover an ICS, whereas \sysname only took 0.5 to 17 minutes.

Figure ~\ref{fig:eval:RQ2} (a) depicts the logarithmic-scaled time distribution of DriveFuzz and \sysname in discovering $12$ ICSs only detected by DriveFuzz. 
Overall, the maximum discovery time \sysname uses is 3x shorter than the minimum discovery time DriveFuzz takes.
Furthermore, DriveFuzz exhibits relatively 20x larger median times than \sysname for detecting these ICSs. 
When examining the average computation time, \sysname still maintains a significant advantage.
Regardless of the type of the ICSs, DriveFuzz consistently requires 20\textasciitilde70x longer discovery time compared to \sysname as illustrated in Figure~\ref{fig:eval:drivefuzz_ave_times}.
The substantial disparity in computation time suggests that starting from the non-collision scenario space incurs a significant amount of additional exploration time, which is unproductive for discovering ICSs.







The developers have confirmed all the detected ICSs, with a partial of them fixed swiftly.
One of the ICSs has also been assigned the corresponding CVE ID due to its potential threats for real-world ADS.\footnote{The CVE number will be exposed after the paper review.}
Furthermore, within the discovered ICSs, we have identified another category of scenarios referred to as IC-prone scenarios, which arise due to the over-conservative behavior of our oracle (discussed in \S~\ref{sec:eval:rq4_oracle-threshold}).
IC-prone scenarios encompass situations where the distance between the vehicle and other traffic participants is extremely close but without actual collisions.
Due to its explicit threats to pedestrians and bicycles, we do not exclude them from ICSs discovered in DriveFuzz and \sysname.
The total number and proportion of IC-prone scenarios can be calculated using the precision obtained in \S~\ref{sec:eval:rq4_oracle-threshold}.
In the following comparison and analysis, we use the term ICSs to represent both ICSs and IC-prone scenarios.
%also include the CVE; more explanation why the IC-prone scenarios are important

\begin{tcolorbox}
\textbf{Answer to RQ1:} 
\sysname can effectively detect ICSs compared with the state-of-the-art approaches. We outperform existing efforts to detect 2.3x more ICS issues with a 20-70x speedup, including high-impact vulnerability and a new type of security issue with CVE assigned.
\end{tcolorbox}


%proportion


%explain the result. data, type, comparison
% number; type; and time 


%impact: cve+ic-prone(definition and description)



\begin{comment}
    
% The primary objective of \sysname is to effectively discover all ICSs.
Therefore, we compare the discovery speed of \sysname with other ADS fuzzers regarding the time needed for discovering ICSs.
Since the oracle used by DriveFuzz is the default collision detector in the simulator, to compare DriveFuzz with \sysname, the oracle used by DriveFuzz was replaced by an IC-oriented oracle as introduced in \S~\ref{sec:overview}.
During a 36-hour runtime of IC-capable DriveFuzz, it executed a total of 779 times and successfully identified 12 ICS cases across three ICS categories, which are 6 ICS 03, 1 ICS 05, and 5 ICS 09, as listed in Table~\ref{tab:discovered_ICs}.

The time for DriveFuzz listed in Table ~\ref{tab:discovered_ICs} is the average time spent identifying the ICSs of the corresponding category.
Due to the limited number of ICSs discovered by DriveFuzz, the proportion for DriveFuzz in Table ~\ref{tab:discovered_ICs} includes both ICS and IC-prone scenarios.
Notably, there are significant differences in both time and proportion compared with \sysname.
While \sysname takes approximately 0.5-20 minutes to find an ICS, DriveFuzz requires an average of 0.5-3.3 hours.
Furthermore, despite considering IC-prone scenarios, there remains a significant difference in the proportion of discovered ICSs between DriveFuzz and \sysname.
The proportion of ICSs discovered by \sysname is much higher than that of DriveFuzz. While DriveFuzz could find a maximum of ICSs accounted for 3\% among all generated scenarios, \sysname could discover up to 40\%.
The disparities in speed and proportion demonstrate the effectiveness and accuracy of \sysname.
In addition, \sysname also identified seven additional types of ICSs that DriveFuzz did not discover.
\end{comment}


%% rq2
% \input{input/float_figs/fig_eval_DriveFuzz_TimeCost}


\begin{comment}
\textbf{Qualitative comparison.}
\wei{different testing target; unsuitable mutation strategy-after analysis the detect result of drivefuzz}
First, the testing target of DriveFuzz is not solely focused on finding collision scenarios.
The goal of the 

It aims to identify scenarios that indICe dangerous behaviors sICh as sudden braking or sharp turns and finally cause illegal events like running red lights, crossing lanes and collisions.
As a result, the number of collision scenarios it discovers may be fewer compared to the fuzzing approach that only focuses on finding collision scenarios.

Second, the EV DriveFuzz tested is equipped with the Autoware ADS or the intelligent driving system in Carla. 
The EV is less likely to exhibit extremely aggressive or rarely occurring driving behaviors.
When using DriveFuzz to test IC events, IC typically occurs at very low speeds(less than 20).
The IC 03 events DriveFuzz found all happened when EV driving at low speed, it may be challenging to identify the same type of IC while EV driving at a high speed.
\end{comment}


\subsection{RQ2: Can \sysname Efficiently Discover ICS Starting From the Collision Scenario Space?}
\label{sec:eval:rq2_search_space}
We further compare \sysname and DriveFuzz to investigate the effectiveness of using collision scenarios to detect ICSs.
Specifically, we evaluate the proportion of discovered ICSs in each type of scenario.

The results can be found in Table~\ref{tab:discovered_ICs}.
\sysname demonstrates a better performance with a minimum proportion of 11.46\% and a maximum of 36.1\%, while DriveFuzz achieves a minimum proportion of 1.03\% and a maximum of 3.08\%.
Even after excluding IC-prone scenarios from the results of \sysname, the proportion of identified ICSs remained 10\textasciitilde20x larger than that of DriveFuzz, as illustrated in Figure~\ref{fig:eval:drivefuzz_ave_times}.
Such a higher proportion rate boosts \sysname to detect all ten types of ICS using less time than DriveFuzz, which only discovered three types of ICSs.
The differences in proportion and type number suggest that initiating the exploration from the non-collision space is less effective in identifying a comprehensive range of ICSs. 
It increases the risk of overlooking ICSs and limits the overall efficiency of the discovery process.

\begin{tcolorbox}
\textbf{Answer to RQ2:} The significant multiple-fold increase in the ICS proportion and a shorter detection time compared to DriveFuzz to discover ICSs demonstrate the effectiveness of starting from the collision space compared with the non-collision space. 
\end{tcolorbox}
% Moreover, another crucial type of dangerous scenario, IC-prone scenarios, have been identified. \wei{keep the last sentence?}


\ignore{
%% rq2: DriveFuzz in 
\input{tables/tab_eval_IC_DriveFuzz}


We also ran DriveFuzz in different modes they offer for 36 hours separately, 
the results are presented in Table~\ref{tab:eval:drivefuzz-IC}. 
DriveFuzz can merely detect a few IC events within the limited runtime regardless of the mode used.
DriveFuzz tends to spend more time exploring the non-collision space than exploring further possibilities within the collision space.
It also stops immediately after finding an IC event and then initiates a new round of testing using a new seed scenario. 
As a result, DriveFuzz not only misses the opportunity to explore the IC space but also spends more time restarting from a new position in non-collision space, which is unrelated to the previous round.
Also, the IC events identified by DriveFuzz, after investing a significant amount of time, exhibit a notable repetition, 
which further highlights the inefficiency of its search strategy.
Comparatively, our incremental search strategy that commences from the collision space has exhibited a discernible superiority.
}


\begin{comment}
We further compared the average computation time taken by DriveFuzz and \sysname to discover different classes of IC events and the proportion that IC events occupy among all detected scenarios. 
Since DriveFuzz only identified three categories of IC events, our comparison focuses on the average time for each of these three types.
% To account for the limited number of IC events discovered by DriveFuzz, IC-prone scenarios found by DriveFuzz are included.
The results, including the time ratio and proportion ratio, are presented in Figure~\ref{fig:drivefuzz_ave_times}.
The time ratio measures how many times the average time taken by DriveFuzz to discover an event within a specific class exceeds the average time taken by ICFuzz.
Notably, for IC 03 and IC 09, the execution time has exceeded 70 times. 
Even though DriveFuzz exhibited a shorter discovery time for IC 05, \sysname demonstrated a speed 20 times faster than DriveFuzz.
The proportion ratio indicates the difference in the proportion of IC events discovered by ICFuzz compared to the proportion of IC-prone events identified by DriveFuzz.
Even when accounting for the IC-prone scenarios identified by DriveFuzz, the proportion of IC events in the results obtained by \sysname was still 10\textasciitilde20 times larger than in DriveFuzz.

Figure~\ref{fig:drivefuzz_time} shows the distribution of time taken to find each IC event.
The minimum amount of time DriveFuzz took for a certain IC event was 17 mins, while the maximum time was 5 hours. 
The average time DriveFuzz took to identify a single IC event is approximately 3 hours, indicating that DriveFuzz required a substantial amount of time to get from non-collision space to collision space.
In contrast, \sysname typically takes 0.5 minutes to 5 minutes to find a IC event, with the longest duration not exceeding 20 minutes.

The analysis of the overall data indicates a higher proportion of instances in the non-collision space.
DriveFuzz tends to spend a longer time exploring the non-collision space instead of exploring further possibilities within the collision space.
The reason is that DriveFuzz stops immediately after finding a IC event and then initiates a new round of testing using a new seed scenario. 
As a result, DriveFuzz misses the opportunity to explore the vicinity of the IC event but also spends more time reverting back to a start position at non-collision space which is unrelated to the previous round.
The IC events identified by DriveFuzz after investing a significant amount of time exhibit a notable repetition, which further highlights the inefficiency of the strategy of finding a IC event and immediately stopping to restart the process.

Besides, since the EV DriveFuzz tested is equipped with an Autoware ADS or the intelligent driving system in Carla. 
The EV is less likely to exhibit extremely aggressive or rarely occurring driving behaviors.
When using DriveFuzz to test IC events, IC typically occurs at a low-speed scope(less than 20).
The IC events DriveFuzz found all happened when the EV driving at low speed, it may be challenging to identify the same type of IC while the EV is driving at a high speed.

%conclusion
The results demonstrate that \sysname outperforms the state-of-the-art ADS fuzzer regarding both detection speed and the proportion of IC events discovered. 
\sysname exhibits a significantly faster discovery speed and a higher proportion of findings, which indicates that starting from the collision space is more effective than starting from the non-collision space.
\end{comment}


%% RQ3: Factor1: IC SR with Collision Distance
\input{input/float_figs/fig_eval_IC_SR_CollisionDistance}




%%
\subsection{\textbf{RQ3:} Can Step-wise Mutation Generate ICSs Effectively?}
\label{sec:eval:rq3_search_direction}

To further study the effectiveness of \sysname, we conduct an ablation evaluation for our step-wise mutation.
The scenarios tested are listed in \S~\ref{sec:emp:scenario_selection}.
The involved parameters are collision distance, speed, and angle, 
whose exact physical meanings are shown in Figure~\ref{figure:control_parameter}. 


\textbf{Collision Distance}: Overall, the data trend in the final result indicates that the effective search direction for ICS searching of collision distance is towards increasing distance in all scenarios except for PCF, where the direction decreases distance.  
In scenario FLB (Figure~\ref{fig:sr_distance-flb}), FLV (Figure~\ref{fig:sr_distance-flv}), LC (Figure~\ref{fig:sr_distance-lc}) and PSF (Figure~\ref{fig:sr_distance-psf}), 
there is a significant positive correlation between ICS SR and collision distance.
Similarly, in scenario InC (Figure~\ref{fig:sr_distance-inc}), the overall SR trend remains, with a slight fluctuation in the middle distance range.
In scenario PCF (Figure~\ref{fig:sr_distance-pcf}), 
the overall ICS SR exhibits a declining trend as the distance increases.
The reason for the negative correlation in scenario PCF is that the NPC pedestrian is walking in the direction perpendicular to the driving direction of the EV.
As the collision distance increases, the probability of the NPC pedestrian moving out of the collision area also increases. 

The overall upward trend aligns with our search direction, and the significant difference in SR observed during the transition from low speed to medium/high speed demonstrates the effectiveness of our search step size.
Moreover, the data trend contradicts the intuition regarding the relationship between collision distances and collisions in reality. 
Intuitively, one would expect a higher occurrence of collisions when two vehicles are close to each other and one of them changes the driving behavior, suggesting that more ICSs should occur within a close distance.
However, the results reveal that more ICSs are found when the distance between two vehicles is far, with one of them altering their driving behavior.




\textbf{Collision Speed}:
The experimental results indicate that, although the collision speed parameter does not significantly impact the overall outcomes compared to the other two parameters, a positive correlation still exists between the ICS success rates and collision speed in most scenarios.
From Figure ~\ref{fig:IC_SR-speed}, it can be observed that in most scenarios, there exists a positive trend between collision speed and the final ICS SR.
Except for FLV, more ICS were discovered while collision speed was at the middle range.

The data illustrates that more ICSs are found when the collision speed is high, which aligns with our search direction and illustrates that our search steps are effective for detecting ICSs.
Our empirical study reveals that, in reality, a higher number of collisions occur at low collision speeds, where one would expect a more significant presence of ICSs. 
However, contrary to this expectation, our experimental results 
are in the opposite direction in most scenarios about the collision factor speed, which demonstrates that more ICSs are found when the collision speed is middle and high. 
The distinction may be because, at high collision speeds, the collision detector lacks sufficient time to react and detect the collision accurately, leading to a higher proportion of ignored collisions.


%% RQ3: Factor2: IC SR with Collision Speed
\input{input/float_figs/fig_eval_IC_SR_CollisionSpeed}



\textbf{Collision Angle}: 
The data trends of ICS SR related to angle in different scenarios align with the trend of high on both sides and low in the middle. 
The fluctuations in the data result from some specific environmental settings.

Overall, for collision angle values greater than 0, a positive correlation between the collision angle and the final ISC SR is observed in almost all scenarios except for scenarios in FLV, indicating its effectiveness in detecting ICS.
The data trend of scenarios in FLV with the positive angle range exhibits fluctuations. 
One reason is that many ICS-prone scenarios mentioned in \S~\ref{sec:eval:rq1_drivefuzz_comparison} happen when the angle is near 0.

For collision angle values smaller than 0, the ICS SR trends of most scenarios also match our conclusion derived from the study, except for PSF and FLV.
For scenario PSF, it does not have ICS when the collision angle is negative since the pedestrian is standing in the right front of the EV.
In scenario FLV, the peak observed in the negative angle range can also be attributed to a higher number of occurrences of type 3 ICS within the specific angle range.
The decreasing trend observed as the collision angle approaches $-1$ is due to the scenarios being at the border between collision and non-collision, leading to a decrease in both the number of collisions and the corresponding number of ICSs.



The search direction for collision angle is from -1 or 1 to 0 ($-90^\circ$ or $90^\circ$ to $0^\circ$ in Figure~\ref{figure:control_parameter}).  
The steep slope of the data trend demonstrates the effectiveness of the search direction and search steps obtained from our study.
However, the collision frequency trend in reality is the opposite; there are more collisions when the collision angle is close to 0, given that the "Vehicle State While Colliding" has the highest proportion of vehicles moving straight ahead.
The reason for such counter-intuition distinction is that collision angles near 0 often result in a stronger collision force, making them less likely to be missed by the collision detector. 
Conversely, collision angles approaching 1 and -1 ($-90^\circ$ and $90^\circ$) encompass a broader range of collision and non-collision scenarios, leading to more identified ICSs.




% \wei{simplify and non-heuristic; the explanation do not related to ICS
% }
% In scenario FLB (Figure~\ref{fig:sr_angle-flb}), LC (Figure~\ref{fig:sr_angle-lc}), and PSF (Figure~\ref{fig:sr_angle-psf}), 
% a notable distinction is observed in the data trend regarding the different representative collision scenarios,
% underscore the necessity of our step-wise mutation.
% In scenario FLB, the number of ICSs with positive collision angles is more significant than those with negative angles,  which is primarily due to the position of the NPC bicycle being slightly right in front of the EV and the small size of the bicycle creating more opportunities for collisions when the collision angle is positive.

% Additionally, more obstacles are on the right side of the road, increasing the likelihood of EV rebounding and creating a secondary collision with the NPC bicycle.
% In scenario LC, the ascending trend of the Angle-SR curve towards both ends shows that, in sideswipe collision scenarios, collisions like ICS No.04 and ICS No.05 involving the corners of the vehicles are more likely to happen compared to other collision situations.
% In scenario PCF, the predominant type of ICS involves the vehicle's side grazing the walking NPC pedestrian, exhibiting a symmetrical data trend.

% In scenario FLV (Figure~\ref{fig:sr_angle-flv}), the trend still roughly follows this pattern, but there are some anomalous fluctuations.
% One possible explanation is that narrower road widths and numerous obstacles on roadsides can lead to multiple subsequent collisions after a single collision.
% The collision in scenario FLV may be detectable by the simulator at first. However, after the struck vehicle hits a roadside barrier and bounces back, the serial second collision with the EV may become an ICS.

% In scenario PSF (Figure~\ref{fig:sr_angle-psf}), since the standing position of the pedestrian is in front of the right side of the EV, only positive collision angles are relevant.
% The opposite data trend can be observed compared to the collision distribution in reality.
% The upward trend in SR as the collision angle increases is the condition that the NPC pedestrian was grazed by the front bumper of the EV when the EV changed its driving behavior using a positive collision angle as ICS 09 in Table~\ref{tab:discovered_ICs}. 
% The peak in the number of ICS observed when the collision angle is approximately 0 is due to type ICS 08. 
% The side of the EV grazed the NPC pedestrian but did not knock it down.
% In scenario InC(Figure~\ref{fig:sr_angle-inc}), a positive collision angle leads to more ICSs. 
% This is attributed to the initial positions of the EV and NPC and their respective driving directions, which consistently intersect within the region represented by the positive collision angle.








% The opposite data trend can also be observed compared to the collision distribution in reality.
% However, the situation is slightly different when the collision angle is negative.
% The number of ICSs decreases when the collision angle increases towards -0.5.
% Therefore, within the range of -1 to -0.5, a better search direction is to start from -1 and decrease the angle to -0.5.
% One potential explanation for the anomalous fluctuations in the data trend is the narrower road width and numerous obstacles on the roadsides, which could result in multiple subsequent collisions following an initial collision.
% The collision in scenario FLV may be a detectable collision at first. 
% Still, after the struck vehicle hits a roadside barrier and bounces back, the collision detector may ignore serial collisions with an EV.


% For the ICS SR, since we started searching from the collision scenario space,
% we avoid generating numerous irrelevant scenarios, resulting in a relatively smaller denominator.
% Together, the success rate is high in some scenarios.
% Moreover, the ICSs we discovered not only help us find different types of ICS but also help us to analyze how different collision-contributing factors affect ICS occurrences. 







%% RQ3: Factor 3: IC SR with Collision Angle
\input{input/float_figs/fig_eval_IC_SR_CollisionAngle}




\begin{tcolorbox}[
float=true,
float=htbp,
]
\noindent \textbf{Answer to RQ3:}
% \wei{the studied factors are useful-> trend is anti-intuition-> explanation-> our method still effective}
The data trends of all three control parameters with their ICS success rate underscore the effectiveness of our empirical study in \S~\ref{sec:emp_study}.
Together with our selected scenarios, we avoid generating numerous irrelevant scenarios to detect ICSs efficiently.
Meanwhile, these general factors also help us to analyze the reason for ICS occurrences. 
Moreover, the trend of discovered ICSs in the simulator is counter-intuitive to collisions in reality.
Such discrepancy highlights the challenge of detecting ICSs with existing efforts and the potential risks that cannot be overlooked.
\end{tcolorbox}



% The data trends for ICSs SR in different representative collision scenarios vary but generally follow similar patterns for each control parameter.
% When analyzing the influence of each control parameter in combination with others, the overall data trends align closely with those observed when considering them individually, without significant deviations. 
% The appendix (\S~\ref{sec:eval:multiple_factor}) analyzes and describes the final ICS success rate when accounting for the combined effects of various control parameters.


% In generally, 
% The effective search direction identified in the results aligns with the search direction when considering the collision angle alone.




%%
% \subsubsection{Ablations}
% \label{eval:rq3-single_feature}

%%
% \smallskip
% \noindent\textbf{Ablations: How does each factor influence the results in different representative collision scenarios? 
% }

% \textbf{Collision Distance}



\begin{comment}
In other positive correlated scenarios, a longer collision distance creates a larger collision zone where the EV has more time and space to adjust its driving behavior.
For example, in scenario FLB, IC 02 primarily occurs at a larger collision distance since a small collision force that sends the NPC bicycle to flying without being detected is more likely to occur at a far collision distance and a low to middle collision speed.

The reason for the negative correlation in scenario PCF\_MOVING is that the NPC pedestrian is walking in the direction perpendicular to the driving direction of EV.
As the collision distance increases, the probability of the NPC pedestrian moving out of the collision area also increases. 
Therefore, the IC SR decreases with an increasing collision distance. 

Due to the longer vehicle body length of cars compared to bicycles and pedestrians, collision accidents where the strICk NPC object is a vehicle are more likely to occur at a larger collision distance as shown in Figure~\ref{fig:sr_distance-flv} and Figure~\ref{fig:sr_distance-flv-h}.
In the case of FLV(see Figure~\ref{fig:sr_distance-flv}) and FLV-H(see Figure~\ref{fig:sr_distance-flv-h}), it is noted that FLV exhibits a higher number of IC occurrences compared to FLV-H in the middle distance scope. 
It can be attributed to the narrower width of the road strICture in scenario FLV and the obstacles on the roadside. 
Consequently, FLV is more susceptible to being hindered by surrounding obstacles after a collision at proximity, leading to subsequent collisions. 
The multiple collisions also contribute to the overall higher number of IC occurrences in FLV compared to FLV-H even the same test step size is used for both scenarios.
\end{comment}


%%


\begin{comment}
In scenario FLB, when the strICk NPC is a bicycle, we observed that the proportion of IC events accounting for all collision events is essentially the same at all speeds as shown in Figure~\ref{fig:sr_speed-flb}. 
The highest number of IC cases occurred within the collision speed range of 5-15, particularly around a collision speed of approximately 8, approximately 4\% to 6\% higher compared to other collision speed values. 


In scenarios FLV(see Figure~\ref{fig:sr_speed-flv}) and FLV-H(see Figure~\ref{fig:sr_speed-flv-H}), the proportion of IC exhibits an initial increase followed by a decreasing trend. 
Even in scenario FLV-H, where the overall proportion of IC is low due to road conditions, this trend is still observed.
Based on our analysis of the data, the reason why the IC sICcess rate is low in the low-speed scope and high-speed speed is that there is a higher number of CD cases and a lower number of IC cases in both two scopes. 
However, there is a lower number of CD cases and a higher number of IC cases at moderate speeds.

In scenarios PCF(see Figure~\ref{fig:sr_speed-pcf}) and PCF\_MOVING(see Figure~\ref{fig:sr_speed-pcf_moving}), where the strICk object is a pedestrian, the proportion of IC increases with higher collision speeds.
We hypothesize that the higher proportion of IC in pedestrian cases at higher speeds is attributed to the increased likelihood of pedestrians being directly knocked away by the collision, resulting in potential missed detections of the collision detection module. 

In scenario IC(see Figure~\ref{fig:sr_speed-ica}), where the collision position changes to the side of the NPC vehicle, the trend becomes positively correlated compared to the rear-end collision condition in scenarios FLV and FLV-H. 
\end{comment}














\begin{comment}
In scenario FLB(see Figure~\ref{fig:sr_angle-flb}), the occurrence of IC events is more frequent when the collision angle is positive or negative.
The number of IC events with positive collision angles is greater than those with negative angles, 
which is primarily due to the position of NPC bicycle being slightly right in front of the EV, and the small size of the bicycle creates more opportunities for collisions when the collision angle is positive.
Additionally, more obstacles are on the right side of the road, increasing the likelihood of EV rebounding and creating a secondary collision with the NPC bicycle.

\wei{explain the FLV}
In scenarios FLV-H(see Figure~\ref{fig:sr_angle-flv-h}), the curve exhibits larger values at both ends and smaller values in the middle. 
The ascending trend of the angle curve towards both ends shows that in read-end vehicle collision scenarios, collisions like IC 04 and IC 05 involving the corners of the vehicles are significantly more compared to other collision situations.
% In scenario FLV, the trend still roughly follows this pattern, but there are some anomalous flICtuations.
% One possible explanation is the narrower road width and the presence of numerous obstacles on roadsides lead to multiple subsequent collisions after a single collision.
% The collision in scenario FLV may be a normal CD event at first, but after the strICk vehicle hits a roadside barrier and bounces back, the serial second collision with EV may become a IC event.

In scenario PCF(see Figure~\ref{fig:sr_angle-pcf}) and PCF\_MOVING(see Figure~\ref{fig:sr_angle-pcf_moving}), there is also an upward trend in SR as the collision angle increases, except when the collision angle is approximately 0.
The NPC pedestrian was grazed by the front bumper of EV when the EV changed its driving behavior using a positive collision angle as IC 09 in Table \ref{tab:discovered_ICs}.
When the collision angle is approximately 0, pedestrians may be grazed by the EV but not knocked down as IC 09 in Table\ref{tab:discovered_ICs}.

In scenario IC(see Figure~\ref{fig:sr_angle-ic}), positive collision angles combined with specific collision speed and collision distance values create IC 06 and IC 07 where the side of NPC vehicle grazed the front or read bumper of EV. 
Negative collision angles often indicate that the NPC vehicle has already driven out of the collision zone, which is caused by the negative angle.
\end{comment}





%% Relationship 3: Distance vs Speed.
% \input{input/float_figs/fig_eval_Relationship1_CollisionDistance_with_Speed}


\ignore{
%%
\subsubsection{Multiple Factors}
\label{sec:eval:rq3_multiple_factor}

\textbf{Q1. Does the search direction for collision speed change at different collision distances?}
From Figure~\ref{fig:IC_SR-distance-speed}, it can be observed that for three specific collision distance groups, there is not a significant variation across different collision speed ranges.
The trend confirms the conclusion drawn in \S~\ref{eval:rq3-single_feature} regarding the limited impact of collision speed as a single feature, indicating that collision speed does not significantly contribute to the search for IC events.


\textbf{Q2. Does the search direction for collision distance change at different collision speed scopes?}
Figure~\ref{fig:IC_SR-speed-distance} shows the trends in the SR across different collision distances for three collision speed scopes.
The observed patterns strongly support the conclusion made in \S~\ref{eval:rq3-single_feature} regarding the impact of collision distance as a single feature.
In most scenarios, except for PCF, the effective search direction indicates increased collision distance.
For PCF, the effective search direction suggests a decrease in collision distance.


\begin{comment}
In scenario FLB(see Figure~\ref{fig:sr-distance-speed-flb}), the number of IC events of middle and far collision distance are both high and higher than the condition that in low collision distance. 
Consistent with the previous findings on the impact of individual factors, a higher occurrence rate of ICs is observed with greater collision distances and low collision speeds.
The decreasing trend between collision speed and IC is observed in the middle to long collision distance scope.
At close collision distance, there is no correlation between collision speed and IC SR, as SR remains relatively constant across different collision speed ranges. 

In scenarios FLV(see Figure~\ref{fig:sr-distance-speed-flv}) and FLV-H(see Figure~\ref{fig:sr-distance-speed-flv-h}), the pattern of collision speed and collision distance observed in the previous section still holds.
Far collision distance and middle-range collision speed create more IC events in scenario FLV.
In FLV-H, the positive correlation between SR, collision distance, and collision speed remains in effect.

In scenario PCF(see Figure~\ref{fig:sr-distance-speed-pcf}), far collision distance and high collision speed lead to high IC occurrences which confirms the separate trend from Figure~\ref{fig:IC_SR-distance} and Figure~\ref{fig:IC_SR-speed}.
The positive correlation does not exist in low collision distance scope, possibly because the collision area is too small and the collision type can not distribute representatively.

In scenario PCF\_MOVING(see Figure~\ref{fig:sr-distance-speed-pcf_moving}), the positive trend holds both low and high.
However, the trend is first upward and then downward in the middle collision distance which cannot be observed in previous figures analyzing a single factor.    

In scenario IC(see Figure~\ref{fig:sr-distance-speed-ic}), the overall trend is consistent with that observed when analyzing individual factors in isolation.
\end{comment}





\textbf{Q3. Does the search direction for collision angle change at different collision speed scopes?}
The relationship between IC occurrences and the collision angle, as depicted in Figure~\ref{fig:IC_SR-speed-angle}, remains mainly unchanged across different collision speed conditions compared to the trend without considering the effect of collision speed shown in Figure~\ref{fig:IC_SR-angle}.
The effective search directions for the collision angle remain consistent across different speed scopes, similar to when considering the collision angle independently. 
In scenario IC, a distinct data trend difference at low collision speed is observed at positive collision angles.
However, since the pattern is not observed in other scenarios, it is likely attributed to data noise.
Even considering the collision angle, the relationship between SR and collision speed is still the same, as shown in Figure~\ref{fig:IC_SR-speed}. 
The observed trends and search directions mentioned above indicate that collision speed does not affect the collision angle either, which further confirms that collision speed does not play a significant role.


% collision speed at different collision distance: almost the same with small flICtuations 


% The SR is the lowest under low collision speed conditions and highest under high collision speed conditions in scenarios FLV-H, PCF, FLV-H, and ICA.



\textbf{Q4. Can \sysname precisely identify all IC events?} 
When considering the variations of collision angle across different collision distances, the observed data trend differs slightly from Figure~\ref{fig:IC_SR-angle}.

In scenarios LC, PSF, and InC, the data aligns with increasing collision angle, bringing more ICSs.
Similarly, although there are fewer fluctuations in the middle collision distance scope in scenario FLV, the overall trend still holds. 
Moreover, the SR exhibits a higher slope at greater collision distances, indicating that simultaneously increasing both collision distance and collision angle can lead to more ICSs.

 
% Relationship 2: Angle vs Speed
% \input{input/float_figs/fig_eval_Relationship2_CollisionAngle_Speed}


In this scenario FLB(see Figure~\ref{fig:sr-dist-angle-flb}), the relationship between collision angle and final SR is unstable and exhibits significant fluctuations under far collision distances. 
The effective search direction for collision angle is increasing the angle to the positive direction at low collision distances.
For middle and far collision distances, the search direction aligns with the overall direction, which involves searching from the middle toward both ends.
Changing driving behavior from a greater collision distance can increase the likelihood of creating secondary collisions, which may explain the fluctuations in middle and far collision distances.


%% Relationship 3: Angle vs Distance
% \input{input/float_figs/fig_eval_Relationship3_CollisionAngle_Distance}


In scenario PCF, exceptions also occur at low collision distances. 
The exception results in different search directions for PCF at different collision distances compared to the one shown in Figure~\ref{fig:sr_angle-pcf}.
In the low collision distance scope, there are hardly any ICSs for the positive collision angle.
Hence, the search direction should be towards increasing negative collision angles.
Conversely, the situation is reversed in the middle and far collision distance scopes.
There are few collision incidents when the collision angle is negative, so the search direction should be towards increasing the positive collision angles.
The significant occurrence of ICSs in the negative collision angle zone at low collision distances can be attributed to the different relative positions between the EV and the NPC if driving behavior changes at different collision distances. 
When driving behavior changes at low collision distances, the pedestrian steps onto the lane, corresponding to the negative collision angle region.
The vehicle must veer towards the negative angle region to collide with the pedestrians.
On the other hand, at middle to high collision distances, the pedestrian has already reached the region marked by the positive collision angle by the time the EV approaches.
Hence, collision events are more likely to occur in this region.


In summary, the effective search direction found in the results aligns with our pre-defined search direction for collision distance.
As for the collision angle, even though there may be fewer ICSs in certain conditions within the positive or negative collision angle ranges, our method of incrementally increasing the search direction from 0 in either positive or negative direction ensures we can still find a sufficient number of ICSs.
}





%%
\subsection{\textbf{RQ4:} Can \sysname Precisely Identify All Detected ICSs?}
\label{sec:eval:rq4_oracle-threshold}


%% OracleThreshold
\input{input/float_figs/fig_eval_OracleThresholdRelationship}

As we use the object detection bounding box as our oracle for ICS discovery, we aim to investigate whether this oracle is sufficiently reliable and accurate in identifying ICSs.
Therefore, we conducted an ablation study to examine the relationship between threshold and performance and investigate the impact of the IoU threshold on the final ICS results.
Three representative scenarios, FLB, LC, and PSF, are tested, each involving different struck objects.
We explore whether different NPC types affect the TP proportion when the IoU threshold changes.
 
For scenario FLB, 
We set the collision distance to 3 and the collision speed to 2. The collision angle on the x-axis was fixed at 0.02, while the collision angle on the y-axis varied from 0 to 1 in increments of 0.02. 
Similarly, for scenario LC, we set the collision distance to 5 and the collision speed to 30. The collision angle on the y-axis was fixed at 0.02, and the collision angle on the y-axis ranged from 0 to 1 with a step of 0.02. 
For scenario PSF, we set the collision distance to 2 and the collision speed to 4. The collision angle on the x-axis was fixed at 0, and the collision angle on the y-axis ranged from 0 to 1 with a step of 0.02. 
Each scenario will be run 50 times under the specification above.
The final results have been manually confirmed and presented in Figure~\ref{fig:oracle_threshold}.


The final precision, recall, and the number of true positives are shown in Figure~\ref{fig:oracle_threshold}.
For scenario FLB, involving a bicycle as the NPC, the precision remains relatively consistent for thresholds ranging from 0 to 0.15. However, the recall decreases as the threshold increases, with a significant drop beyond 0.15. The optimal threshold value for FLB is still 0. 
Similarly, for scenario LC with a vehicle as the NPC, the precision is high at thresholds of 0 and 0.2. However,  there is only 1 TP when the threshold is 0.2, the number of true positives exhibits a decreasing trend, and an IoU threshold of 0 yields the best results. In scenario PSF with a pedestrian as the NPC, raising the threshold above 0.05 did not result in additional ICSs. Therefore, setting the threshold at 0 is still the most reasonable choice for our ICS discovery method.

\ignore{
For scenario FLB, where the NPC is a bicycle, the results are shown in Figure~\ref{fig:oracle_threshold-precision-flb} and Figure \ref{fig:oracle_threshold-num-flb}.
We observed that the precision remains relatively consistent for thresholds ranging from 0 to 0.15. 
However, the recall shows a decreasing trend as the threshold increases
Once the threshold surpasses 0.15, the precision increases but begins to decline, while the recall experiences a sharp drop.
Figure \ref{fig:oracle_threshold-num-flb} also depicts a decrease in true positives (TP) with the increase in the IoU threshold.
The optimal threshold value for scenario FLB is still 0.

The situation is slightly different for scenario FLV-H, where the NPC is a vehicle.
As collisions with a vehicle often result in IC cases where the impact is just a graze without altering the motion state of the strICk object, the recall tends to be lower compared to the FLB scenario.
From Figure \ref{fig:oracle_threshold-precision-flv-h}, the precision is high when the threshold is either 0 or 0.2. 
However, when considering the number of TP shown in Figure \ref{fig:oracle_threshold-num-flv-h}, there is only 1 TP when the threshold equals 0.2.
The recall and threshold are negatively correlated. 
Similar to the FLB scenario, the number of TP exhibits a decreasing trend.
In summary, collisions with a vehicle, similar to collisions with pedestrians, yield the best results with an IoU threshold set to 0.

In scenario PCF, where the NPC is a pedestrian, no additional IC events have occurred since the threshold was raised above 0.05.
Therefore, it is likely that the threshold for the collision detector in Carla is around 0.05.
When the threshold is equal to 0.05, although the precision is high, only one TP is detected. 
For our IC detection method, it is still more reasonable to use the threshold as 0.
}
% \wei{check}
% In conclusion, although our oracle may have some false positives in the threshold we set, \sysname can still effectively detect ICSs.
% Moreover, the false positive results actually have reality meaning be as the IC-prone scenarios.
% They provided new dangerous types of scenario which can be used to guide the further ADS testing.
% The ADS may not have collisions while tested in simulator, but the dangerous scenarios that close to collisions also make them dangerous in reality and threaten the safety of other traffic participants.
% As it is an orthogonal problem to this paper, we will minimize the FP resulting from the bounding box's over-conservative in future work.

\begin{tcolorbox}
\textbf{Answer to RQ4:} Despite the potential false positives in the threshold set for our oracle, \sysname remains highly effective in detecting ICSs according to our empirical evidence.
Additionally, the false positive results may include IC-prone scenarios that hold practical significance, introducing new threats for ADS in real-world scenarios.
\end{tcolorbox}

==> tables/Algorithm.tex <==

\begin{algorithm}
\label{sec:design:algo}
\caption{UCFuzz testing procedure}
\begin{algorithmic}[1]
    \Require $S$ : a set of pre-determined DC scenarios (seed pool), $strategy$ : mutation strategy, $d$ : search direction, $s$ : search step, $N_C$ : maximum \# cycles // \S~\ref{sec:design:offline} %\Statex \qquad 
    \Ensure $UC_s$ : recorded UC events, $s'$ : UC-prone scenarios 
    
    \Function {UC\_Testing}{$seed$}
        \State $s \gets seed$
        \State $s' \gets mutator.mutate(s,\ strategy,\ d,\ seed)$ //\S~\ref{sec:design:mutator}
        
        \For { $cycles \gets$ 1 $to$ $N_C$ }
            % \State $s' \gets mutator.generate(s, strategy, d, s)$
            \State $results, states = detector.check\_uc(executor.simulate(s'))$ //\S~\ref{sec:design:detector}
            % \State $results \gets executor.simulate(s')$
            % \State $states \gets detector.check\_uc(results)$
            \If{$results == True$}
                \State $UC_s \gets save\_UC\_events(states,s')$
            \ElsIf{$states == Non-Collision$}
                \State $NC\_Count++$ 
            \EndIf
            \If{$NC\_Count>NC\_Threshold$}
                \State \Return
            \EndIf
            \State $s' = mutator.mutate(s, strategy, d, s)$
        \EndFor
    \EndFunction 

    % \ForEach 
    \ForEach
    {$s \in \mathcal S $}
        \State UC\_Testing(seed)
    \EndFor  
\end{algorithmic}
\end{algorithm}


==> tables/algo_Mutater.tex <==
%% 
\begin{algorithm}[tp]
% \label{alg_mutator}
\caption{ICFuzz Mutator}
\label{algo:algo_mutator}
%% 
\begin{algorithmic}[1]
\Require Scenario $scenario$: \{"Angle": $\hat{\theta}$, "Speed": $\hat{v}$, "Distance": $d$, ...\},
Control Factor $factor$: \{$name, direction, stepsize$\},

% \\
% $direction$: \{+, -\} $factor$ , 
% \\
% $stepsize$: $factor$
\Ensure scenario
\Function {Mutate}{$scenario$, $factor$}
    \State $\delta$ $\gets$ $factor.direction$ $\times$  $factor.stepsize$
    \State $scenario[factor.name]$ $\gets$ $scenario[factor.name]$ + $\delta$
    \State \Return $scenario$
\EndFunction
\end{algorithmic}
\end{algorithm}


==> tables/tab_CollisionTypes.tex <==
%%
% \captionsetup{labelfont=bf}
% \captionsetup{font=bf}
\begin{table}[tp]
\centering
\caption{Percentage of the highest number of collision types for Autonomous Vehicles(AVs) and Convolutional Vehicles(CVs)}
\resizebox{\columnwidth}{!}{ %
% \begin{tabular}{@{}lll@{}}
\begin{tabular}{lcc}
\toprule
% \begin{tabular}[c]{@{}l@{}}Collision Types\\ dgsdgg\end{tabular}
\textbf{Collision Types}
& \textbf{CVs(\%)} 
& \textbf{AVs(\%)}
\\ 
\midrule
Leading vehicle stopped 
& 21.2   
& 31.15   
\\
Vehicle Change Lanes(same direction)
& 9.21    
& 13.15   
\\
Leading Vehicle Decelerating     
& 7.39   
& 16.39   
\\
Vehicle Turing at Non-Signalized Junction                       
& 11.47   
& 9.02    
\\
Running red light                                                
& 8.11    
& 2.46    
\\
Left Turn Across Path from Opposite Directions at Signalized Junction \zk{too long}
& 10.7    
& /       
\\ 
\bottomrule
\end{tabular}%
}
\label{tab: AV_Collision_scenarios}
\end{table}


==> tables/tab_CrashFactors.tex <==
%% 
\begin{table}[tp]
\centering
\caption{Collision Factors.}
%% resize the entire tabular
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{|c|c|l|}
%% 
\toprule
%% header
\textbf{\makecell{Crash \\ Factors}}
& \textbf{Target}
& \textbf{Values}
\\
\hline
\midrule


%% factor: Time
\parbox[t]{0pt}{
\multirow{7}{*}{
    \rotatebox[origin=c]{90}{
        \textbf{Time}
    }
}
}
& \multirow{4}{*}[0pt]{AV}
& \makecell[l]{
    Daylight (43.75\%),
    Dark (56.25\%)
    ~\cite{divergent_effect}
} 
\\
\cline{3-3}
% -
& % -
& \makecell[l]{
    Daylight (67.3\%),   
    Unknown (32.7\%)
    ~\cite{avoid}
} 
\\
\cline{3-3}
% -
& % -
& \makecell[l]{
    Daylight (64.52\%), 
    Dark street lights (33.33\%),  
    \\
    Dusk-dawn (2.15\%)
    ~\cite{analysis_poi}
}
\\
\cline{3-3}
% -
& % -
& \makecell[l]{
    Daylight (45\%),     
    Other (43\%),   
    % \\
    Dark night (9\%),    
    Dusk-dawn (3\%)
    ~\cite{automated_latent}
} 
\\
\cline{2-3}
% -
& \multirow{3}{*}[5pt]{Bicycle}
& \makecell[l]{
    Good daytime lighting (46.4\%), 
    Poor daytime lighting (15.4\%),
    \\
    Poor lighting at night  (28.5\%),  
    Poor lighting at night (9.7\%)
    ~\cite{car-bicycle_analysis}
}
\\
\cline{3-3}
% -
& % - Bicycle
& \makecell[l]{  
    Daylight (52.2\%),
    Dark (30.1\%),
    Dusk or Dawn (17.8\%)
    ~\cite{single_bicycle_crash}
} 
\\
\cline{3-3}
% -
& % Bicycle
& \makecell[l]{
    Daytime (77.2\%),
    Nighttime w/ Lighting (18.3\%),
    \\
    Nighttime wo/ Lighting (4.5\%)
    ~\cite{identifying_factors}
} 
\\
\midrule
%% end Time


%% factor: collision type
\parbox[t]{4pt}{
\multirow{7}{*}[-50pt]{
    \rotatebox[origin=c]{90}{
        \textbf{\makecell{Collision Type}}
    }
}
}
& \multirow{6}{*}[-10pt]{AV}
& \makecell[l]{
    Rear-end: (59.38\%), 
    Other (40.63\%) 
    ~\cite{divergent_effect}
}
\\
\cline{3-3}
% -
& % AV
& \makecell[l]{
    Front (25.7\%),  
    Left (25.1\%),  
    Rear (21.2\%),
    Right (21\%),
    \\
    Top (4.5\%), 
    Bottom (2.4\%)
    ~\cite{avoid}
}  
\\
\cline{3-3}
% -
& % AV
& \makecell[l]{
    Rear-end (64\%), 
    Sideswipe (15\%), 
    Broadside (12\%),
    Head-on (12\%)
    ~\cite{analysis_poi}
}
\\
\cline{3-3}
% -
& % AV
& \makecell[l]{
    Rear-end (61.1\%),  
    Sideswipe (24.8\%), 
    Other (6.2\%), 
    \\
    Broadside (5.3\%), 
    Head-on (2.7\%)
    ~\cite{exploratory_cal}
} 
\\
\cline{3-3}
% -
& % AV
& \makecell[l]{
    Rear-end (49.85\%),  
    Sideswipe (20.64\%),
    Head-on (10.86\%), 
    \\
    Broadside (6.57\%), 
    Bike/Pedestrian (6.7\%),  
    Hit object (5.81\%)
    ~\cite{learn_crash}
}
\\
\cline{3-3}
% -
& % AV
& \makecell[l]{
    Other (45\%),  
    Rear-end (38\%),    
    Sideswipe (11\%),  
    \\
    Head-on (3\%),
    Hit-object (3\%)
    ~\cite{automated_latent}
} 
\\
\cline{2-3}
% -
& Pedestrian
& \makecell[l]{
    Frontal impact (43.8\%), 
    Side impact (24.1\%),  
    \\
    Car moving forward (23.2\%),
    Back (6.2\%),
    No impact (3.6\%)
    ~\cite{typical_pedestrian}
} 
\\
\cline{2-3}
% -
& \multirow{4}{*}{Bicycle}
& \makecell[l]{
    For bicycle:
    Side (54.7\%),
    Frontal (19.9\%), 
    \\
    Scrape (14.2\%),
    Rear-end (8.2\%), 
    Others (3\%), 
    \\
    For vehicle: 
    Left hood (24.3\%),
    \\
    Frontal hood (17.6\%),
    Right hood (26.7\%),
    \\
    Left back (4.1\%),
    Back (3\%),
    Right back (2.6\%), 
    \\
    Left body (9.7\%),
    Right body (12\%)
    ~\cite{car-bicycle_analysis}
} 
\\
\cline{3-3}
% -
& % Bicycle
& \makecell[l]{
    Front (64.4\%),  
    Right (19.4\%), 
    Left (10.6\%),  
    Rear (5.6\%)
    ~\cite{identifying_factors}
} 
\\
\midrule
%% end Collision Type


%% factor: Speed
\parbox[t]{4pt}{
\multirow{4}{*}{
    \rotatebox[origin=c]{90}{
        \textbf{Speed}
    }
}
}
& \multirow{2}{*}{AV}
& \makecell[l]{
    % speed limit:   
    \textless{}=25mph (88.54\%),  
    \textgreater{}25mph (21.88\%)
    ~\cite{divergent_effect}
} 
\\
\cline{3-3}
% -
& % AV
& \makecell[l]{
    {[}0,15{]} (31.8\%), 
    {[}15,30{]} (17.3\%), 
    {[}30,45{]} (16.2\%),
    \\
    {[}45,60{]} (16.2\%), 
    {[}60.75{]} (15\%), 
    {[}75,90{]} (2.9\%), 
    {[}90,105{]} (0.6\%)
    m/s
    ~\cite{avoid}
} 
\\
\cline{2-3}
% -
& Pedestrian
& \makecell[l]{
    % vehicle speed: 
    2-10m/s (50.8\%),
    10-20m/s (42.9\%), 
    \\
    20-30m/s (5.9\%),
    \textgreater{} 30m/s (0.5\%)
    ~\cite{pedestrian_causation}
} 
\\
\cline{2-3}
% -
& Bicycle
& Speeding (33.1\%)~\cite{car-bicycle_analysis}
\\
\midrule
%% end Speed


%% factor: Weather
\parbox[t]{0pt}{
\multirow{7}{*}{
    \rotatebox[origin=c]{90}{
        \textbf{Weather}
    }
}
}
& \multirow{3}{*}{AV}
& \makecell[l]{
    Clear weather (88.54\%),  
    Cloudy (5.21\%) ,   
    \\
    Raining (3.13\%),  
    Fig/Visibility (2.08\%)
    ~\cite{divergent_effect}
} 
\\
\cline{3-3}
% -
& % AV
& \makecell[l]{
    Clear (77.42\%), 
    Cloudy (19.35\%), 
    % \\
    Raining (12.15\%),
    Fog (1.08\%)
    ~\cite{analysis_poi}
} 
\\
\cline{3-3}
% -
& % AV
& \makecell[l]{
    Clear(48\%),
    Other(44\%),
    % \\
    Cloudy(5\%), 
    Raining(2\%), 
    Fog(1\%)
    ~\cite{automated_latent}
} 
\\
\cline{2-3}
% -
& \multirow{4}{*}{Bicycle}
& \makecell[l]{
    Sunny (70.87\%),
    Rain (15.72\%), 
    Fog (7.11\%),
    \\
    Snow (2.6\%),
    Rain (3.7\%)
    ~\cite{car-bicycle_analysis}
} 
\\
\cline{3-3}
% -
& % Bicycle
& \makecell[l]{
    Clear (68.9\%), 
    Rain/Snow/Fog (16.7\%),  
    Cloudy (14.4\%)
    ~\cite{identifying_factors}
} 
\\
\cline{3-3}
% -
& % Bicycle
& \makecell[l]{
    Visibility fine (82.8\%),
    Visibility reduced (14.9\%), 
    Other (2.3\%)
    ~\cite{single_bicycle_crash}
} 
\\
\midrule
%% end Weather


%% factor: Accident Location
\parbox[t]{0pt}{
\multirow{7}{*}[-20pt]{
    \rotatebox[origin=c]{90}{
        \textbf{Accident Location}
    }
}
}
& \multirow{5}{*}{AV}
& \makecell[l]{
    Road Type:
    Intersection (65.63\%)
    \\
    Street Width:
    \textless{}=60 feet(78.13\%)
    % \\
    Trees: 80.21\% 
    ~\cite{divergent_effect}
} 
\\
\cline{3-3}
% -
& % AV
& \makecell[l]{
    Highway/Freeway (32.0\%), 
    Unknown (37.6\%), 
    Intersection (13.6\%),
    \\
    Street (13.4\%), 
    Rural road (2.2\%),
    % \\
    Parking lot (1.3\%)
    ~\cite{avoid}
} 
\\
\cline{3-3}
% -
& % AV
& \makecell[l]{
    Intersection (47.31\%), 
    Street (35.48\%),  
    \\
    Highway (13.98\%),  
    Parking lot (3.23\%)
    ~\cite{analysis_poi}
}
\\
\cline{3-3}
% -
& % AV
& Intersection (73.5\%)~\cite{exploratory_cal}
\\
\cline{3-3}
% -
& % AV
& \makecell[l]{
    Intersections (69.72\%),    
    Street (21.71\%),     
    Expressway (4.74\%)
    ~\cite{learn_crash}
} 
\\
\cline{2-3}
% -
& \multirow{2}{*}{Bicycle}
& \makecell[l]{
    Road Type:
    Straight road (23.9\%),  
    \\
    Ramp (9.4\%),
    Four-leg intersection (45.6\%),  
    \\
    Three-leg intersection (21.1\%), 
    Single-lane (5.6\%),  
    \\
    Two-lane two-way (7.8\%), 
    Four-lane two-way (24.4\%),  
    \\
    Six-lane, two-way (62.2\%), 
    \\
    Road condition:
    Dry (78.9\%),  
    Wet (16.7\%),
    Water (4.4\%)
    ~\cite{identifying_factors}
} 
\\
\cline{3-3}
% -
& % Bicycle
& \makecell[l]{
    Urban (79\%), 
    Rural (21\%)  
    % \\
    Road condition:
    Dry road surface (31\%),
    \\
    Slippery (49.6\%),
    Wet (18.9\%)
    ~\cite{single_bicycle_crash}
} 
\\
\midrule
%% end Accident Location



%% factor: Vehicle State While Collide.
\parbox[t]{5pt}{
\multirow{6}{*}[-20pt]{
    \rotatebox[origin=c]{90}{
        \textbf{\makecell{Vehicle State}}
    }
}
}
& \multirow{5}{*}[-20pt]{AV}
& \makecell[l]{
    Straight  (87.50\%),
    Turning movement (12.50\%)
    ~\cite{divergent_effect}
} 
\\
\cline{3-3}
% -
& % AV
& \makecell[l]{
    Other (36.63\%),  
    Proceeding straight (20.89\%), 
    Unknown (19.89\%),  
    \\
    Left turn (4.95\%),  
    Changing lanes (4.41\%), 
    \\
    Right turn (1.98\%),  
    Backing (1.89\%)
    ~\cite{avoid}
}   
\\
\cline{3-3}
% -
& % AV
& \makecell[l]{
    Stopped (36.08\%),  
    Proceeding straight (29.9\%),
    Right turn (5.15\%), 
    \\
    Slowing/Stopping (10.31\%),
    Left turn (4.12\%), 
    \\
    Changing lanes (4.12\%),  
    Parking maneuver (2.06\%)
    ~\cite{analysis_poi}
}  
\\
\cline{3-3}
% -
& % AV
& \makecell[l]{
    Left turn (11.5\%),  
    Right turn (21.2\%),
    No turning (66.3\%)
    ~\cite{exploratory_cal}
}  
\\
\cline{3-3}
% -
& % AV
& \makecell[l]{
    Other (44.64\%),  
    Stopped (23.21\%),  
    Straight (15.18\%), 
    \\
    Left turn (3.57\%), 
    Right turn (2.68\%)
    ~\cite{automated_latent}
}  
\\
\cline{2-3}
% -
& Pedestrian
& \makecell[l]{
    Vehicle moving forwards  (99.11\%), 
    Parked or reversing  (0.89\%)
    ~\cite{typical_pedestrian}
} 
\\
\midrule
%% end Vehicle State While Collide.


%% factor: Collide With
\parbox[t]{5pt}{
\multirow{2}{*}{
    \rotatebox[origin=l]{90}{
        \textbf{\makecell{Collide \\ With}}
    }
}
}
& AV
& \makecell[l]{
    Non-motor vehicles or 
    pedestrians involved (18.75\%)
    ~\cite{divergent_effect}
}
\\
\cline{2-3}
% 
& Pedestrian
& \makecell[l]{
    Car/taxi (90.88\%),
    Motorcycle (3.97\%),
    Bus (5.97\%),
    \\
    Light goods vehicle (1.95\%), 
    Other (2.09\%),
    \\
    Pedal cycle (1.48\%),
    Unknown vehicle(0.06\%) 
    ~\cite{typical_pedestrian}
}
\\
\midrule
%% end Collide With


%% factor: # of vehicle 
\parbox[t]{5pt}{
\multirow{3}{*}{
    \rotatebox[origin=l]{90}{
        \textbf{\makecell{\# of \\ Vehicles}}
    }
}
}
& \multirow{3}{*}{AV}
& \makecell[l]{
    2 (87.50\%),
    1 (11.46\%),   
    3 (1.04\%)
    ~\cite{divergent_effect}
} 
\\
\cline{3-3}
% -
& % -
& \makecell[l]{
    2: (90.3\%),  
    1 (8\%),  
    3 (1.8\%)
    ~\cite{exploratory_cal}
} 
\\
\cline{3-3}
% -
& % - 
& \makecell[l]{
    2 (84.16\%),  
    1 (12.87\%), 
    Multi (1.97\%)
    ~\cite{automated_latent}
}
\\
% \midrule
%% end # of vehicle 
%% 
\bottomrule
\end{tabular}
}
\label{tab:design:CrashFactors_all}
\end{table}


==> tables/tab_CrashFactors_values.tex <==
%% 
\begin{table}[tp]
\centering
%% Resize the entire tabular
\resizebox{0.45\textwidth}{!}{
%% 
\begin{tabular}{|c|l|}
%% 
\toprule
%% header
\makecell[c]{Target}
& Crash Scenarios
\\
\midrule
%% 
AV
& 
\makecell[l]{
AV maneuvers while NPC proceeds straight;
\\
NPC rule violation;
\\
NPC maneuvers while AV proceeding straight;
\\
AV collided with a fixed object;
\\
AV stopped and hit by NPC 
}
\\
\midrule
%%
AV
&
\makecell[l]{
From most to least:
\\
1. Head on/rear end + Two vehicles collision + Fog/Cloudy
\\
2. Two Moving Vehicles + Clear Weather + Weekdays 
\\
+ Daylight
\\
2. Side swipe + Left / Right turn / Straight as prior event
\\
+ Weekdays + Dark
\\
4. Single Vehicle Crash
\\
5. Multi-Vehicle + Moving 
}
\\
\midrule
%% 
AV 
&
\makecell[l]{
Relationship between scenario and collision severity:
\\
1. T-shaped intersection + NPC proceeding straight 
\\
+ Wet Road Surface -> No Injury
\\
2. Un-signalized Intersection + 14:00-16:00 -> Light Injury
\\
3. AV + NPC Lane Change -> Moderate Damage Crashes
\\
4. Intersection + AV + Light Weather + Dry Road 
\\
-> Moderate Crashes
\\
5. Non-Signalized Intersection + AV + Wet Road Surface  
\\
+ Large Vehicles -> Severe Injuries
}
\\
\midrule
%% 
Bicycle
&
\makecell[l]{
a. 
Front(initial contact area) + Clear Weather + Daytime
\\
+ Four-Leg Intersection + Six-Lane Two-Way + Dry Road 
\\
b. Left + Clear Weather + Daytime + Four-Leg Intersection 
\\
+ Six-Lane Two-Way + Dry Road
\\
c. Front + Clear Weather + Daytime + Four-Leg Intersection 
\\
+ Four Lane Two-Way + Wet Road 
\\
d. Front + Clear Weather + Night Time With Lighting
\\
+ Straight Road+ Six-Lane Two-Way + Dry Road   
\\
e. Front + Clear Weather + Daytime + Three-Leg Intersection 
\\
+ Six-Lane Two-Way + Dry road + Visual Obstruction
\\
f. Right + Clear Weather + Daytime + Four-Leg Intersection 
\\
+ Ramp + Dry Road 
}
\\
\midrule
%% 
Pedestrian
&
\makecell[l]{
1. Vehicle going straight, Pedestrian crossing the road \\ without obstacles. (49.86\%)
\\
2. Vehicle going straight, Pedestrian walking along the road \\ (or standing still) without obstacles. (23.96\%)
\\
3. Vehicle going straight and Pedestrian crossing
the road \\ with obstacles. (13.37\%)
\\
4. Vehicle turning and Pedestrian crossing the road \\ at an intersection without obstacles. (8.08\%)
\\
5. Vehicle backing up and Pedestrian crossing \\
the road without obstacles. (4.74\%)
}
\\
%% 
\bottomrule
\end{tabular}
}
\caption{TODO:}
\label{tab:CrashFactorsValues}
\end{table}


==> tables/tab_TestedScenarios.tex <==
%%
\begin{table}[tp]
\caption{Collision-prone scenarios for testing. Features are the collision-related factors we aim to investigate regarding their influence on the occurrence of ICEs.}
\label{tab:tested_scenarios}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccc@{}}
\toprule
Scenario    & Abbr  & Struck Object Type    & Features                             
\\ 
\midrule
Follow Leading Bicycle  & FLB   & Bicycle   & O 
\\
Follow Leading Vehicle  & FLV   & Vehicle   & O
\\
Lane Change  & LC & Vehicle   & O, R
\\
Intersection Collision & Inter-C & Vehicle & O, P                                 
\\
Pedestrian Standing Front & PSF & Pedestrian & O                                    
\\
Pedestrian Crossing Front & PCF & Pedestrian & O, M                                 
\\ 
\midrule
\multicolumn{4}{l}{
    \begin{tabular}[c]{@{}l@{}}
    [Impact Features] \textbf{O}: StrICEk Object Type, \textbf{R}: Road Type, \textbf{P}: Collision Position,  
    \\ 
    \textbf{M}: Motion Status of the StrICEk Object
    \end{tabular}
} 
\\ 
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/tab_TopCollisionTypes.tex <==
%%
% \captionsetup{labelfont=bf}
% \captionsetup{font=bf}
\begin{table}[tp]
\centering
\caption{The prevalent collision types account for over 5\% of Autonomous Vehicles(AVs). The CVs column represents the proportion of the corresponding collision types with the collision accidents involving only Convolutional Vehicles(CVs).}
\resizebox{1.0\columnwidth}{!}{ %
% \begin{tabular}{@{}lll@{}}
\begin{tabular}{clccc}
% \begin{tabular}{|p{1.5cm}|p{1.5cm}}

\toprule
% \begin{tabular}[c]{@{}l@{}}Collision Types\\ dgsdgg\end{tabular}
\textbf{No.}
& \textbf{Collision Types}
& \textbf{AVs(\%)}
& \textbf{CVs(\%)} 
& \textbf{Collision Results}
\\ 
\midrule
1
& Leading vehicle stopped  
& 31.15   
& 21.2  
& RE
\\
2
& Vehicle Change Lanes (same direction)
& 18.85 
& 9.21  
& CC / SS

\\
3
& Leading Vehicle Decelerating     
& 16.39   
& 7.39   
& RE
\\
4
& Vehicle Turning at Non-Signalized Junction
& 14.76
& 11.47  
& RE / SS
\\
5
& Following Vehicle Making a Maneuver
& 5.74
& 0.91
& RE / CC / SS
% \\
% \bottomrule
\\ 
\midrule
\multicolumn{3}{l}{
    \begin{tabular}[c]{@{}l@{}}
    [Collision Results] \textbf{RE}: Read-End, \textbf{CC}: Corner Collision, \textbf{SS}: Sideswipe,  
    \end{tabular}
} 
\\ 
\bottomrule

\end{tabular}%
}
\label{tab: AV_Collision_scenarios}
\end{table}




==> tables/tab_eval_DrivingParameters.tex <==
%%
\begin{table}[tp]
\centering
\caption{Control parameters to be adjusted during testing. \zk{Not that necessary. To be merged into Figure~\ref{figure:control_parameter}}}
\label{tab:driving_parameters_table}
\resizebox{\columnwidth}{!}{
% \begin{tabular}{@{}ll@{}}
\begin{tabular}{c|l}
\toprule
\textbf{Notation} 
& \textbf{Definition}

\\
\midrule
$d$
& 
\makecell[l]{Collision Distance. Distance threshold between ego vehicle and another actor. \\ When it is reached, change the driving behavior of EV.}
% \begin{tabular}[c]{@{}l@{}}Distance threshold between ego vehicle and another actor. \\ When it is reached, change the driving behavior of the ego vehicle.\end{tabular} 
\\
\midrule
$\hat{v}$          
& Collision Speed. The sustained driving speed of EV after changing driving behavior.
\\
$\hat{\theta}$  
& Collision Angle. Driving angle of EV after changing driving behavior. $\hat{\theta} = <\hat{\theta}_{x}, \hat{\theta}_{y}>$  
\\                            
$\hat{\theta}_{x}$  
& Projection of the collision angle on the x-axis.                                                            
\\
$\hat{\theta}_{y}$  & Projection of the collision angle on the y-axis.                               
\\ 
\bottomrule
\end{tabular}
}
\end{table}




\begin{comment}

%%
\begin{table}[tp]
\centering
\caption{Driving Parameters \wei{add explanation os adjustment}}
\label{tab:driving_parameters_table}
\resizebox{\columnwidth}{!}{
% \begin{tabular}{@{}ll@{}}
\begin{tabular}{c|l}
\toprule
\textbf{Notation} 
& \textbf{Definition}
\\ 
\midrule
$v$           
& Initial driving speed of ego vehicle                                
\\
$\theta_{x}$ 
& Initial driving angle on the x-axis of the ego vehicle                   
\\
$\theta_{y}$   
& Initial driving angle on the y-axis of the ego vehicle   
\\
\midrule
$d$
& 
\makecell[l]{Collision Distance. Distance threshold between ego vehicle and another actor. \\ When it is reached, change the driving behavior of EV.}
% \begin{tabular}[c]{@{}l@{}}Distance threshold between ego vehicle and another actor. \\ When it is reached, change the driving behavior of the ego vehicle.\end{tabular} 
\\
\midrule
$\hat{v}$          
& Collision Speed. The sustained driving speed of EV after changing driving behavior.
\\
$\hat{\theta}$  
& Collision Angle. Driving angle of EV after changing driving behavior. 
\\                            
$\hat{\theta}_{x}$  
& Projection of the collision angle on the x-axis.                                                            
\\
$\hat{\theta}_{y}$  & Projection of the collision angle on the y-axis.                               
\\ 
\bottomrule
\end{tabular}
}
\end{table}
\end{comment}

==> tables/tab_eval_IC_DriveFuzz.tex <==
%%
\begin{table}[tp]
\centering
\caption{\S~\ref{sec:appdenix:2}: The number of ICSs identified by DriveFuzz}
\label{tab:eval:drivefuzz-IC}
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{c|cccc}
\toprule
\textbf{Mutation Mode} & \textbf{All}  & \textbf{Congestion} & \textbf{Entropy} & \textbf{Instability} 
\\ 
\midrule
Running times & 779 & 884        & 1976    & 893   
\\
Detected ICS  & 12   & 10         & 22      & 0 
\\ 
\bottomrule
\end{tabular}%
}
\end{table}
